Single-Scanline Relative Pose Estimation for Rolling Shutter Cameras

We propose a novel approach for estimating the relative pose between rolling shutter cameras using the intersections of line projections with a single scanline per image. This allows pose estimation without explicitly modeling camera motion. Alternatively, scanlines can be selected within a single image, enabling single-view relative pose estimation for scanlines of rolling shutter cameras. Our approach is designed as a foundational building block for rolling shutter structure-from-motion (SfM), where no motion model is required, and each scanline's pose can be computed independently. % We classify minimal solvers for this problem in both generic and specialized settings, including cases with parallel lines and known gravity direction, assuming known intrinsics and no lens distortion. Furthermore, we develop minimal solvers for the parallel-lines scenario, both with and without gravity priors, by leveraging connections between this problem and the estimation of 2D structure from 1D cameras. % Experiments on rolling shutter images from the Fastec dataset demonstrate the feasibility of our approach for initializing rolling shutter SfM, highlighting its potential for further development. % The code will be made publicly available.

==> Figs/stability_rotation.tex <==
\begin{axis}[%
xmode=log,
width=0.25\columnwidth,
height=0.16\columnwidth,
at={(1.0in,0.389in)},
scale only axis,
xmin=1e-18,
xmax=10,
xlabel style={font=\color{white!15!black}},
xlabel={Rot err (rad)},
ymin=0,
ymax=15000,
ytick={0,10000},
xtick={1e-6,1e-15},
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
%ylabel style={yshift=-0.15in},
%ylabel={Frequency},
legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=6
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=red,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.334050268600027769e-20 0.000000000000000000e+00 \\
2.225329969703585113e-20 0.000000000000000000e+00 \\
3.712074117909952463e-20 0.000000000000000000e+00 \\
6.192112830212035034e-20 0.000000000000000000e+00 \\
1.032906673848005283e-19 0.000000000000000000e+00 \\
1.722992177523380382e-19 0.000000000000000000e+00 \\
2.874124176918259319e-19 0.000000000000000000e+00 \\
4.794328083497031032e-19 0.000000000000000000e+00 \\
7.997421251594711528e-19 0.000000000000000000e+00 \\
1.334050268600027926e-18 0.000000000000000000e+00 \\
2.225329969703585089e-18 0.000000000000000000e+00 \\
3.712074117909952560e-18 0.000000000000000000e+00 \\
6.192112830212034649e-18 0.000000000000000000e+00 \\
1.032906673848005355e-17 0.000000000000000000e+00 \\
1.722992177523380305e-17 0.000000000000000000e+00 \\
2.874124176918259049e-17 0.000000000000000000e+00 \\
4.794328083497030300e-17 2.000000000000000000e+00 \\
7.997421251594709602e-17 4.000000000000000000e+00 \\
1.334050268600027833e-16 1.600000000000000000e+01 \\
2.225329969703590759e-16 5.800000000000000000e+01 \\
3.712074117909949355e-16 3.040000000000000000e+02 \\
6.192112830212025928e-16 8.350000000000000000e+02 \\
1.032906673848005379e-15 1.784000000000000000e+03 \\
1.722992177523380280e-15 3.385000000000000000e+03 \\
2.874124176918252048e-15 5.420000000000000000e+03 \\
4.794328083497023053e-15 7.618000000000000000e+03 \\
7.997421251594710194e-15 9.566000000000000000e+03 \\
1.334050268600027883e-14 1.063200000000000000e+04 \\
2.225329969703585099e-14 1.099600000000000000e+04 \\
3.712074117909943596e-14 1.019700000000000000e+04 \\
6.192112830212024824e-14 8.856000000000000000e+03 \\
1.032906673848005253e-13 7.439000000000000000e+03 \\
1.722992177523380249e-13 5.953000000000000000e+03 \\
2.874124176918251795e-13 4.448000000000000000e+03 \\
4.794328083497023747e-13 3.344000000000000000e+03 \\
7.997421251594709689e-13 2.476000000000000000e+03 \\
1.334050268600027782e-12 1.824000000000000000e+03 \\
2.225329969703590564e-12 1.274000000000000000e+03 \\
3.712074117909949327e-12 9.370000000000000000e+02 \\
6.192112830212025429e-12 7.430000000000000000e+02 \\
1.032906673848005339e-11 5.050000000000000000e+02 \\
1.722992177523380047e-11 3.680000000000000000e+02 \\
2.874124176918251573e-11 2.570000000000000000e+02 \\
4.794328083497010580e-11 1.680000000000000000e+02 \\
7.997421251594699026e-11 1.390000000000000000e+02 \\
1.334050268600027960e-10 1.010000000000000000e+02 \\
2.225329969703590920e-10 9.200000000000000000e+01 \\
3.712074117909949650e-10 5.400000000000000000e+01 \\
6.192112830212009726e-10 5.600000000000000000e+01 \\
1.032906673848003633e-09 2.500000000000000000e+01 \\
1.722992177523380150e-09 3.100000000000000000e+01 \\
2.874124176918251780e-09 1.400000000000000000e+01 \\
4.794328083497010735e-09 2.300000000000000000e+01 \\
7.997421251594698199e-09 7.000000000000000000e+00 \\
1.334050268600027794e-08 8.000000000000000000e+00 \\
2.225329969703584995e-08 1.000000000000000000e+01 \\
3.712074117909943777e-08 5.000000000000000000e+00 \\
6.192112830212008568e-08 7.000000000000000000e+00 \\
1.032906673848003625e-07 4.000000000000000000e+00 \\
1.722992177523380448e-07 1.000000000000000000e+00 \\
2.874124176918251548e-07 3.000000000000000000e+00 \\
4.794328083497010669e-07 4.000000000000000000e+00 \\
7.997421251594698001e-07 0.000000000000000000e+00 \\
1.334050268600027847e-06 1.000000000000000000e+00 \\
2.225329969703585246e-06 1.000000000000000000e+00 \\
3.712074117909943380e-06 2.000000000000000000e+00 \\
6.192112830212009521e-06 0.000000000000000000e+00 \\
1.032906673848003662e-05 0.000000000000000000e+00 \\
1.722992177523380300e-05 2.000000000000000000e+00 \\
2.874124176918251570e-05 0.000000000000000000e+00 \\
4.794328083497011135e-05 1.000000000000000000e+00 \\
7.997421251594698255e-05 0.000000000000000000e+00 \\
1.334050268600027889e-04 0.000000000000000000e+00 \\
2.225329969703584857e-04 0.000000000000000000e+00 \\
3.712074117909933656e-04 0.000000000000000000e+00 \\
6.192112830212015721e-04 0.000000000000000000e+00 \\
1.032906673848005275e-03 0.000000000000000000e+00 \\
1.722992177523380124e-03 0.000000000000000000e+00 \\
2.874124176918244414e-03 0.000000000000000000e+00 \\
4.794328083497016203e-03 0.000000000000000000e+00 \\
7.997421251594711428e-03 0.000000000000000000e+00 \\
1.334050268600027803e-02 0.000000000000000000e+00 \\
2.225329969703584987e-02 0.000000000000000000e+00 \\
3.712074117909934523e-02 0.000000000000000000e+00 \\
6.192112830212015417e-02 0.000000000000000000e+00 \\
1.032906673848005275e-01 0.000000000000000000e+00 \\
1.722992177523380297e-01 0.000000000000000000e+00 \\
2.874124176918244622e-01 0.000000000000000000e+00 \\
4.794328083496991466e-01 0.000000000000000000e+00 \\
7.997421251594685199e-01 0.000000000000000000e+00 \\
1.334050268600027955e+00 0.000000000000000000e+00 \\
2.225329969703584876e+00 0.000000000000000000e+00 \\
3.712074117909933690e+00 0.000000000000000000e+00 \\
6.192112830212015417e+00 0.000000000000000000e+00 \\
1.032906673848005141e+01 0.000000000000000000e+00 \\
1.722992177523380164e+01 0.000000000000000000e+00 \\
2.874124176918244444e+01 0.000000000000000000e+00 \\
4.794328083496991155e+01 0.000000000000000000e+00 \\
7.997421251594685998e+01 0.000000000000000000e+00 \\
};
\addlegendentry{$(E,3,5)$}


\addplot [color=green,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.334050268600027769e-20 0.000000000000000000e+00 \\
2.225329969703585113e-20 0.000000000000000000e+00 \\
3.712074117909952463e-20 0.000000000000000000e+00 \\
6.192112830212035034e-20 0.000000000000000000e+00 \\
1.032906673848005283e-19 0.000000000000000000e+00 \\
1.722992177523380382e-19 0.000000000000000000e+00 \\
2.874124176918259319e-19 0.000000000000000000e+00 \\
4.794328083497031032e-19 0.000000000000000000e+00 \\
7.997421251594711528e-19 0.000000000000000000e+00 \\
1.334050268600027926e-18 0.000000000000000000e+00 \\
2.225329969703585089e-18 0.000000000000000000e+00 \\
3.712074117909952560e-18 0.000000000000000000e+00 \\
6.192112830212034649e-18 0.000000000000000000e+00 \\
1.032906673848005355e-17 0.000000000000000000e+00 \\
1.722992177523380305e-17 0.000000000000000000e+00 \\
2.874124176918259049e-17 0.000000000000000000e+00 \\
4.794328083497030300e-17 0.000000000000000000e+00 \\
7.997421251594709602e-17 0.000000000000000000e+00 \\
1.334050268600027833e-16 0.000000000000000000e+00 \\
2.225329969703590759e-16 2.000000000000000000e+00 \\
3.712074117909949355e-16 1.300000000000000000e+01 \\
6.192112830212025928e-16 6.600000000000000000e+01 \\
1.032906673848005379e-15 2.730000000000000000e+02 \\
1.722992177523380280e-15 9.400000000000000000e+02 \\
2.874124176918252048e-15 2.155000000000000000e+03 \\
4.794328083497023053e-15 4.202000000000000000e+03 \\
7.997421251594710194e-15 6.776000000000000000e+03 \\
1.334050268600027883e-14 9.468000000000000000e+03 \\
2.225329969703585099e-14 1.140400000000000000e+04 \\
3.712074117909943596e-14 1.204500000000000000e+04 \\
6.192112830212024824e-14 1.150000000000000000e+04 \\
1.032906673848005253e-13 1.031400000000000000e+04 \\
1.722992177523380249e-13 8.442000000000000000e+03 \\
2.874124176918251795e-13 6.746000000000000000e+03 \\
4.794328083497023747e-13 5.036000000000000000e+03 \\
7.997421251594709689e-13 3.527000000000000000e+03 \\
1.334050268600027782e-12 2.415000000000000000e+03 \\
2.225329969703590564e-12 1.590000000000000000e+03 \\
3.712074117909949327e-12 1.110000000000000000e+03 \\
6.192112830212025429e-12 7.080000000000000000e+02 \\
1.032906673848005339e-11 4.660000000000000000e+02 \\
1.722992177523380047e-11 2.810000000000000000e+02 \\
2.874124176918251573e-11 1.940000000000000000e+02 \\
4.794328083497010580e-11 1.200000000000000000e+02 \\
7.997421251594699026e-11 6.800000000000000000e+01 \\
1.334050268600027960e-10 6.000000000000000000e+01 \\
2.225329969703590920e-10 2.800000000000000000e+01 \\
3.712074117909949650e-10 1.900000000000000000e+01 \\
6.192112830212009726e-10 1.400000000000000000e+01 \\
1.032906673848003633e-09 7.000000000000000000e+00 \\
1.722992177523380150e-09 6.000000000000000000e+00 \\
2.874124176918251780e-09 2.000000000000000000e+00 \\
4.794328083497010735e-09 3.000000000000000000e+00 \\
7.997421251594698199e-09 0.000000000000000000e+00 \\
1.334050268600027794e-08 0.000000000000000000e+00 \\
2.225329969703584995e-08 0.000000000000000000e+00 \\
3.712074117909943777e-08 0.000000000000000000e+00 \\
6.192112830212008568e-08 0.000000000000000000e+00 \\
1.032906673848003625e-07 0.000000000000000000e+00 \\
1.722992177523380448e-07 0.000000000000000000e+00 \\
2.874124176918251548e-07 0.000000000000000000e+00 \\
4.794328083497010669e-07 0.000000000000000000e+00 \\
7.997421251594698001e-07 0.000000000000000000e+00 \\
1.334050268600027847e-06 0.000000000000000000e+00 \\
2.225329969703585246e-06 0.000000000000000000e+00 \\
3.712074117909943380e-06 0.000000000000000000e+00 \\
6.192112830212009521e-06 0.000000000000000000e+00 \\
1.032906673848003662e-05 0.000000000000000000e+00 \\
1.722992177523380300e-05 0.000000000000000000e+00 \\
2.874124176918251570e-05 0.000000000000000000e+00 \\
4.794328083497011135e-05 0.000000000000000000e+00 \\
7.997421251594698255e-05 0.000000000000000000e+00 \\
1.334050268600027889e-04 0.000000000000000000e+00 \\
2.225329969703584857e-04 0.000000000000000000e+00 \\
3.712074117909933656e-04 0.000000000000000000e+00 \\
6.192112830212015721e-04 0.000000000000000000e+00 \\
1.032906673848005275e-03 0.000000000000000000e+00 \\
1.722992177523380124e-03 0.000000000000000000e+00 \\
2.874124176918244414e-03 0.000000000000000000e+00 \\
4.794328083497016203e-03 0.000000000000000000e+00 \\
7.997421251594711428e-03 0.000000000000000000e+00 \\
1.334050268600027803e-02 0.000000000000000000e+00 \\
2.225329969703584987e-02 0.000000000000000000e+00 \\
3.712074117909934523e-02 0.000000000000000000e+00 \\
6.192112830212015417e-02 0.000000000000000000e+00 \\
1.032906673848005275e-01 0.000000000000000000e+00 \\
1.722992177523380297e-01 0.000000000000000000e+00 \\
2.874124176918244622e-01 0.000000000000000000e+00 \\
4.794328083496991466e-01 0.000000000000000000e+00 \\
7.997421251594685199e-01 0.000000000000000000e+00 \\
1.334050268600027955e+00 0.000000000000000000e+00 \\
2.225329969703584876e+00 0.000000000000000000e+00 \\
3.712074117909933690e+00 0.000000000000000000e+00 \\
6.192112830212015417e+00 0.000000000000000000e+00 \\
1.032906673848005141e+01 0.000000000000000000e+00 \\
1.722992177523380164e+01 0.000000000000000000e+00 \\
2.874124176918244444e+01 0.000000000000000000e+00 \\
4.794328083496991155e+01 0.000000000000000000e+00 \\
7.997421251594685998e+01 0.000000000000000000e+00 \\
};
\addlegendentry{$(E,4,4)$}

\addplot [color=blue,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.334050268600027769e-20 0.000000000000000000e+00 \\
2.225329969703585113e-20 0.000000000000000000e+00 \\
3.712074117909952463e-20 0.000000000000000000e+00 \\
6.192112830212035034e-20 0.000000000000000000e+00 \\
1.032906673848005283e-19 0.000000000000000000e+00 \\
1.722992177523380382e-19 0.000000000000000000e+00 \\
2.874124176918259319e-19 0.000000000000000000e+00 \\
4.794328083497031032e-19 0.000000000000000000e+00 \\
7.997421251594711528e-19 0.000000000000000000e+00 \\
1.334050268600027926e-18 0.000000000000000000e+00 \\
2.225329969703585089e-18 0.000000000000000000e+00 \\
3.712074117909952560e-18 0.000000000000000000e+00 \\
6.192112830212034649e-18 0.000000000000000000e+00 \\
1.032906673848005355e-17 0.000000000000000000e+00 \\
1.722992177523380305e-17 0.000000000000000000e+00 \\
2.874124176918259049e-17 0.000000000000000000e+00 \\
4.794328083497030300e-17 0.000000000000000000e+00 \\
7.997421251594709602e-17 0.000000000000000000e+00 \\
1.334050268600027833e-16 0.000000000000000000e+00 \\
2.225329969703590759e-16 0.000000000000000000e+00 \\
3.712074117909949355e-16 0.000000000000000000e+00 \\
6.192112830212025928e-16 1.000000000000000000e+00 \\
1.032906673848005379e-15 7.000000000000000000e+00 \\
1.722992177523380280e-15 3.400000000000000000e+01 \\
2.874124176918252048e-15 1.240000000000000000e+02 \\
4.794328083497023053e-15 2.640000000000000000e+02 \\
7.997421251594710194e-15 5.440000000000000000e+02 \\
1.334050268600027883e-14 8.760000000000000000e+02 \\
2.225329969703585099e-14 1.358000000000000000e+03 \\
3.712074117909943596e-14 1.908000000000000000e+03 \\
6.192112830212024824e-14 2.490000000000000000e+03 \\
1.032906673848005253e-13 2.989000000000000000e+03 \\
1.722992177523380249e-13 3.369000000000000000e+03 \\
2.874124176918251795e-13 3.704000000000000000e+03 \\
4.794328083497023747e-13 3.798000000000000000e+03 \\
7.997421251594709689e-13 3.987000000000000000e+03 \\
1.334050268600027782e-12 3.858000000000000000e+03 \\
2.225329969703590564e-12 3.863000000000000000e+03 \\
3.712074117909949327e-12 3.778000000000000000e+03 \\
6.192112830212025429e-12 3.783000000000000000e+03 \\
1.032906673848005339e-11 3.672000000000000000e+03 \\
1.722992177523380047e-11 3.570000000000000000e+03 \\
2.874124176918251573e-11 3.641000000000000000e+03 \\
4.794328083497010580e-11 3.637000000000000000e+03 \\
7.997421251594699026e-11 3.536000000000000000e+03 \\
1.334050268600027960e-10 3.655000000000000000e+03 \\
2.225329969703590920e-10 3.598000000000000000e+03 \\
3.712074117909949650e-10 3.816000000000000000e+03 \\
6.192112830212009726e-10 3.984000000000000000e+03 \\
1.032906673848003633e-09 3.983000000000000000e+03 \\
1.722992177523380150e-09 3.972000000000000000e+03 \\
2.874124176918251780e-09 3.767000000000000000e+03 \\
4.794328083497010735e-09 3.398000000000000000e+03 \\
7.997421251594698199e-09 2.840000000000000000e+03 \\
1.334050268600027794e-08 2.114000000000000000e+03 \\
2.225329969703584995e-08 1.550000000000000000e+03 \\
3.712074117909943777e-08 1.094000000000000000e+03 \\
6.192112830212008568e-08 6.760000000000000000e+02 \\
1.032906673848003625e-07 3.900000000000000000e+02 \\
1.722992177523380448e-07 2.780000000000000000e+02 \\
2.874124176918251548e-07 1.840000000000000000e+02 \\
4.794328083497010669e-07 1.110000000000000000e+02 \\
7.997421251594698001e-07 7.100000000000000000e+01 \\
1.334050268600027847e-06 4.800000000000000000e+01 \\
2.225329969703585246e-06 4.400000000000000000e+01 \\
3.712074117909943380e-06 2.100000000000000000e+01 \\
6.192112830212009521e-06 2.100000000000000000e+01 \\
1.032906673848003662e-05 1.000000000000000000e+01 \\
1.722992177523380300e-05 8.000000000000000000e+00 \\
2.874124176918251570e-05 8.000000000000000000e+00 \\
4.794328083497011135e-05 4.000000000000000000e+00 \\
7.997421251594698255e-05 0.000000000000000000e+00 \\
1.334050268600027889e-04 0.000000000000000000e+00 \\
2.225329969703584857e-04 0.000000000000000000e+00 \\
3.712074117909933656e-04 0.000000000000000000e+00 \\
6.192112830212015721e-04 2.000000000000000000e+00 \\
1.032906673848005275e-03 1.000000000000000000e+00 \\
1.722992177523380124e-03 1.000000000000000000e+00 \\
2.874124176918244414e-03 3.000000000000000000e+00 \\
4.794328083497016203e-03 5.000000000000000000e+00 \\
7.997421251594711428e-03 7.000000000000000000e+00 \\
1.334050268600027803e-02 1.600000000000000000e+01 \\
2.225329969703584987e-02 3.000000000000000000e+01 \\
3.712074117909934523e-02 4.300000000000000000e+01 \\
6.192112830212015417e-02 6.500000000000000000e+01 \\
1.032906673848005275e-01 1.000000000000000000e+02 \\
1.722992177523380297e-01 1.990000000000000000e+02 \\
2.874124176918244622e-01 2.720000000000000000e+02 \\
4.794328083496991466e-01 3.050000000000000000e+02 \\
7.997421251594685199e-01 3.510000000000000000e+02 \\
1.334050268600027955e+00 1.620000000000000000e+02 \\
2.225329969703584876e+00 2.000000000000000000e+00 \\
3.712074117909933690e+00 0.000000000000000000e+00 \\
6.192112830212015417e+00 0.000000000000000000e+00 \\
1.032906673848005141e+01 0.000000000000000000e+00 \\
1.722992177523380164e+01 0.000000000000000000e+00 \\
2.874124176918244444e+01 0.000000000000000000e+00 \\
4.794328083496991155e+01 0.000000000000000000e+00 \\
7.997421251594685998e+01 0.000000000000000000e+00 \\
};
\addlegendentry{$(D,3,7)$}


\legend{}

\end{axis}

==> Figs/stability_translation.tex <==
\begin{axis}[%
xmode=log,
width=0.25\columnwidth,
height=0.16\columnwidth,
at={(2.0in,0.389in)},
scale only axis,
xmin=1e-11,
xmax=10,
xlabel style={font=\color{white!15!black}},
xlabel={Tran err (rad)},
ymin=0,
ymax=60000,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
%ylabel style={yshift=-0.15in},
%ylabel={Frequency},
legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=6
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=red,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.334050268600027769e-20 0.000000000000000000e+00 \\
2.225329969703585113e-20 0.000000000000000000e+00 \\
3.712074117909952463e-20 0.000000000000000000e+00 \\
6.192112830212035034e-20 0.000000000000000000e+00 \\
1.032906673848005283e-19 0.000000000000000000e+00 \\
1.722992177523380382e-19 0.000000000000000000e+00 \\
2.874124176918259319e-19 0.000000000000000000e+00 \\
4.794328083497031032e-19 0.000000000000000000e+00 \\
7.997421251594711528e-19 0.000000000000000000e+00 \\
1.334050268600027926e-18 0.000000000000000000e+00 \\
2.225329969703585089e-18 0.000000000000000000e+00 \\
3.712074117909952560e-18 0.000000000000000000e+00 \\
6.192112830212034649e-18 0.000000000000000000e+00 \\
1.032906673848005355e-17 0.000000000000000000e+00 \\
1.722992177523380305e-17 0.000000000000000000e+00 \\
2.874124176918259049e-17 0.000000000000000000e+00 \\
4.794328083497030300e-17 0.000000000000000000e+00 \\
7.997421251594709602e-17 0.000000000000000000e+00 \\
1.334050268600027833e-16 0.000000000000000000e+00 \\
2.225329969703590759e-16 0.000000000000000000e+00 \\
3.712074117909949355e-16 0.000000000000000000e+00 \\
6.192112830212025928e-16 0.000000000000000000e+00 \\
1.032906673848005379e-15 0.000000000000000000e+00 \\
1.722992177523380280e-15 0.000000000000000000e+00 \\
2.874124176918252048e-15 0.000000000000000000e+00 \\
4.794328083497023053e-15 0.000000000000000000e+00 \\
7.997421251594710194e-15 0.000000000000000000e+00 \\
1.334050268600027883e-14 0.000000000000000000e+00 \\
2.225329969703585099e-14 0.000000000000000000e+00 \\
3.712074117909943596e-14 0.000000000000000000e+00 \\
6.192112830212024824e-14 0.000000000000000000e+00 \\
1.032906673848005253e-13 0.000000000000000000e+00 \\
1.722992177523380249e-13 0.000000000000000000e+00 \\
2.874124176918251795e-13 0.000000000000000000e+00 \\
4.794328083497023747e-13 0.000000000000000000e+00 \\
7.997421251594709689e-13 0.000000000000000000e+00 \\
1.334050268600027782e-12 0.000000000000000000e+00 \\
2.225329969703590564e-12 0.000000000000000000e+00 \\
3.712074117909949327e-12 0.000000000000000000e+00 \\
6.192112830212025429e-12 0.000000000000000000e+00 \\
1.032906673848005339e-11 0.000000000000000000e+00 \\
1.722992177523380047e-11 0.000000000000000000e+00 \\
2.874124176918251573e-11 0.000000000000000000e+00 \\
4.794328083497010580e-11 0.000000000000000000e+00 \\
7.997421251594699026e-11 0.000000000000000000e+00 \\
1.334050268600027960e-10 0.000000000000000000e+00 \\
2.225329969703590920e-10 0.000000000000000000e+00 \\
3.712074117909949650e-10 2.000000000000000000e+00 \\
6.192112830212009726e-10 2.000000000000000000e+00 \\
1.032906673848003633e-09 1.400000000000000000e+01 \\
1.722992177523380150e-09 1.730000000000000000e+02 \\
2.874124176918251780e-09 1.093000000000000000e+03 \\
4.794328083497010735e-09 7.844000000000000000e+03 \\
7.997421251594698199e-09 4.300000000000000000e+04 \\
1.334050268600027794e-08 4.761300000000000000e+04 \\
2.225329969703584995e-08 2.230000000000000000e+02 \\
3.712074117909943777e-08 7.000000000000000000e+00 \\
6.192112830212008568e-08 7.000000000000000000e+00 \\
1.032906673848003625e-07 6.000000000000000000e+00 \\
1.722992177523380448e-07 2.000000000000000000e+00 \\
2.874124176918251548e-07 2.000000000000000000e+00 \\
4.794328083497010669e-07 3.000000000000000000e+00 \\
7.997421251594698001e-07 3.000000000000000000e+00 \\
1.334050268600027847e-06 0.000000000000000000e+00 \\
2.225329969703585246e-06 3.000000000000000000e+00 \\
3.712074117909943380e-06 0.000000000000000000e+00 \\
6.192112830212009521e-06 0.000000000000000000e+00 \\
1.032906673848003662e-05 1.000000000000000000e+00 \\
1.722992177523380300e-05 0.000000000000000000e+00 \\
2.874124176918251570e-05 1.000000000000000000e+00 \\
4.794328083497011135e-05 1.000000000000000000e+00 \\
7.997421251594698255e-05 0.000000000000000000e+00 \\
1.334050268600027889e-04 0.000000000000000000e+00 \\
2.225329969703584857e-04 0.000000000000000000e+00 \\
3.712074117909933656e-04 0.000000000000000000e+00 \\
6.192112830212015721e-04 0.000000000000000000e+00 \\
1.032906673848005275e-03 0.000000000000000000e+00 \\
1.722992177523380124e-03 0.000000000000000000e+00 \\
2.874124176918244414e-03 0.000000000000000000e+00 \\
4.794328083497016203e-03 0.000000000000000000e+00 \\
7.997421251594711428e-03 0.000000000000000000e+00 \\
1.334050268600027803e-02 0.000000000000000000e+00 \\
2.225329969703584987e-02 0.000000000000000000e+00 \\
3.712074117909934523e-02 0.000000000000000000e+00 \\
6.192112830212015417e-02 0.000000000000000000e+00 \\
1.032906673848005275e-01 0.000000000000000000e+00 \\
1.722992177523380297e-01 0.000000000000000000e+00 \\
2.874124176918244622e-01 0.000000000000000000e+00 \\
4.794328083496991466e-01 0.000000000000000000e+00 \\
7.997421251594685199e-01 0.000000000000000000e+00 \\
1.334050268600027955e+00 0.000000000000000000e+00 \\
2.225329969703584876e+00 0.000000000000000000e+00 \\
3.712074117909933690e+00 0.000000000000000000e+00 \\
6.192112830212015417e+00 0.000000000000000000e+00 \\
1.032906673848005141e+01 0.000000000000000000e+00 \\
1.722992177523380164e+01 0.000000000000000000e+00 \\
2.874124176918244444e+01 0.000000000000000000e+00 \\
4.794328083496991155e+01 0.000000000000000000e+00 \\
7.997421251594685998e+01 0.000000000000000000e+00 \\
};
\addlegendentry{$(E,3,5)$}

\addplot [color=green,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.334050268600027769e-20 0.000000000000000000e+00 \\
2.225329969703585113e-20 0.000000000000000000e+00 \\
3.712074117909952463e-20 0.000000000000000000e+00 \\
6.192112830212035034e-20 0.000000000000000000e+00 \\
1.032906673848005283e-19 0.000000000000000000e+00 \\
1.722992177523380382e-19 0.000000000000000000e+00 \\
2.874124176918259319e-19 0.000000000000000000e+00 \\
4.794328083497031032e-19 0.000000000000000000e+00 \\
7.997421251594711528e-19 0.000000000000000000e+00 \\
1.334050268600027926e-18 0.000000000000000000e+00 \\
2.225329969703585089e-18 0.000000000000000000e+00 \\
3.712074117909952560e-18 0.000000000000000000e+00 \\
6.192112830212034649e-18 0.000000000000000000e+00 \\
1.032906673848005355e-17 0.000000000000000000e+00 \\
1.722992177523380305e-17 0.000000000000000000e+00 \\
2.874124176918259049e-17 0.000000000000000000e+00 \\
4.794328083497030300e-17 0.000000000000000000e+00 \\
7.997421251594709602e-17 0.000000000000000000e+00 \\
1.334050268600027833e-16 0.000000000000000000e+00 \\
2.225329969703590759e-16 0.000000000000000000e+00 \\
3.712074117909949355e-16 0.000000000000000000e+00 \\
6.192112830212025928e-16 0.000000000000000000e+00 \\
1.032906673848005379e-15 0.000000000000000000e+00 \\
1.722992177523380280e-15 0.000000000000000000e+00 \\
2.874124176918252048e-15 0.000000000000000000e+00 \\
4.794328083497023053e-15 0.000000000000000000e+00 \\
7.997421251594710194e-15 0.000000000000000000e+00 \\
1.334050268600027883e-14 0.000000000000000000e+00 \\
2.225329969703585099e-14 0.000000000000000000e+00 \\
3.712074117909943596e-14 0.000000000000000000e+00 \\
6.192112830212024824e-14 0.000000000000000000e+00 \\
1.032906673848005253e-13 0.000000000000000000e+00 \\
1.722992177523380249e-13 0.000000000000000000e+00 \\
2.874124176918251795e-13 0.000000000000000000e+00 \\
4.794328083497023747e-13 0.000000000000000000e+00 \\
7.997421251594709689e-13 0.000000000000000000e+00 \\
1.334050268600027782e-12 0.000000000000000000e+00 \\
2.225329969703590564e-12 0.000000000000000000e+00 \\
3.712074117909949327e-12 0.000000000000000000e+00 \\
6.192112830212025429e-12 0.000000000000000000e+00 \\
1.032906673848005339e-11 0.000000000000000000e+00 \\
1.722992177523380047e-11 0.000000000000000000e+00 \\
2.874124176918251573e-11 0.000000000000000000e+00 \\
4.794328083497010580e-11 0.000000000000000000e+00 \\
7.997421251594699026e-11 0.000000000000000000e+00 \\
1.334050268600027960e-10 0.000000000000000000e+00 \\
2.225329969703590920e-10 0.000000000000000000e+00 \\
3.712074117909949650e-10 0.000000000000000000e+00 \\
6.192112830212009726e-10 0.000000000000000000e+00 \\
1.032906673848003633e-09 1.000000000000000000e+00 \\
1.722992177523380150e-09 1.000000000000000000e+00 \\
2.874124176918251780e-09 1.200000000000000000e+02 \\
4.794328083497010735e-09 2.687000000000000000e+03 \\
7.997421251594698199e-09 3.553900000000000000e+04 \\
1.334050268600027794e-08 6.134300000000000000e+04 \\
2.225329969703584995e-08 2.950000000000000000e+02 \\
3.712074117909943777e-08 5.000000000000000000e+00 \\
6.192112830212008568e-08 4.000000000000000000e+00 \\
1.032906673848003625e-07 0.000000000000000000e+00 \\
1.722992177523380448e-07 3.000000000000000000e+00 \\
2.874124176918251548e-07 1.000000000000000000e+00 \\
4.794328083497010669e-07 1.000000000000000000e+00 \\
7.997421251594698001e-07 0.000000000000000000e+00 \\
1.334050268600027847e-06 0.000000000000000000e+00 \\
2.225329969703585246e-06 0.000000000000000000e+00 \\
3.712074117909943380e-06 0.000000000000000000e+00 \\
6.192112830212009521e-06 0.000000000000000000e+00 \\
1.032906673848003662e-05 0.000000000000000000e+00 \\
1.722992177523380300e-05 0.000000000000000000e+00 \\
2.874124176918251570e-05 0.000000000000000000e+00 \\
4.794328083497011135e-05 0.000000000000000000e+00 \\
7.997421251594698255e-05 0.000000000000000000e+00 \\
1.334050268600027889e-04 0.000000000000000000e+00 \\
2.225329969703584857e-04 0.000000000000000000e+00 \\
3.712074117909933656e-04 0.000000000000000000e+00 \\
6.192112830212015721e-04 0.000000000000000000e+00 \\
1.032906673848005275e-03 0.000000000000000000e+00 \\
1.722992177523380124e-03 0.000000000000000000e+00 \\
2.874124176918244414e-03 0.000000000000000000e+00 \\
4.794328083497016203e-03 0.000000000000000000e+00 \\
7.997421251594711428e-03 0.000000000000000000e+00 \\
1.334050268600027803e-02 0.000000000000000000e+00 \\
2.225329969703584987e-02 0.000000000000000000e+00 \\
3.712074117909934523e-02 0.000000000000000000e+00 \\
6.192112830212015417e-02 0.000000000000000000e+00 \\
1.032906673848005275e-01 0.000000000000000000e+00 \\
1.722992177523380297e-01 0.000000000000000000e+00 \\
2.874124176918244622e-01 0.000000000000000000e+00 \\
4.794328083496991466e-01 0.000000000000000000e+00 \\
7.997421251594685199e-01 0.000000000000000000e+00 \\
1.334050268600027955e+00 0.000000000000000000e+00 \\
2.225329969703584876e+00 0.000000000000000000e+00 \\
3.712074117909933690e+00 0.000000000000000000e+00 \\
6.192112830212015417e+00 0.000000000000000000e+00 \\
1.032906673848005141e+01 0.000000000000000000e+00 \\
1.722992177523380164e+01 0.000000000000000000e+00 \\
2.874124176918244444e+01 0.000000000000000000e+00 \\
4.794328083496991155e+01 0.000000000000000000e+00 \\
7.997421251594685998e+01 0.000000000000000000e+00 \\
};
\addlegendentry{$(E,4,4)$}

\addplot [color=blue,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.334050268600027769e-20 0.000000000000000000e+00 \\
2.225329969703585113e-20 0.000000000000000000e+00 \\
3.712074117909952463e-20 0.000000000000000000e+00 \\
6.192112830212035034e-20 0.000000000000000000e+00 \\
1.032906673848005283e-19 0.000000000000000000e+00 \\
1.722992177523380382e-19 0.000000000000000000e+00 \\
2.874124176918259319e-19 0.000000000000000000e+00 \\
4.794328083497031032e-19 0.000000000000000000e+00 \\
7.997421251594711528e-19 0.000000000000000000e+00 \\
1.334050268600027926e-18 0.000000000000000000e+00 \\
2.225329969703585089e-18 0.000000000000000000e+00 \\
3.712074117909952560e-18 0.000000000000000000e+00 \\
6.192112830212034649e-18 0.000000000000000000e+00 \\
1.032906673848005355e-17 0.000000000000000000e+00 \\
1.722992177523380305e-17 0.000000000000000000e+00 \\
2.874124176918259049e-17 0.000000000000000000e+00 \\
4.794328083497030300e-17 0.000000000000000000e+00 \\
7.997421251594709602e-17 0.000000000000000000e+00 \\
1.334050268600027833e-16 0.000000000000000000e+00 \\
2.225329969703590759e-16 0.000000000000000000e+00 \\
3.712074117909949355e-16 0.000000000000000000e+00 \\
6.192112830212025928e-16 0.000000000000000000e+00 \\
1.032906673848005379e-15 0.000000000000000000e+00 \\
1.722992177523380280e-15 0.000000000000000000e+00 \\
2.874124176918252048e-15 0.000000000000000000e+00 \\
4.794328083497023053e-15 0.000000000000000000e+00 \\
7.997421251594710194e-15 0.000000000000000000e+00 \\
1.334050268600027883e-14 0.000000000000000000e+00 \\
2.225329969703585099e-14 0.000000000000000000e+00 \\
3.712074117909943596e-14 0.000000000000000000e+00 \\
6.192112830212024824e-14 0.000000000000000000e+00 \\
1.032906673848005253e-13 0.000000000000000000e+00 \\
1.722992177523380249e-13 0.000000000000000000e+00 \\
2.874124176918251795e-13 0.000000000000000000e+00 \\
4.794328083497023747e-13 0.000000000000000000e+00 \\
7.997421251594709689e-13 0.000000000000000000e+00 \\
1.334050268600027782e-12 0.000000000000000000e+00 \\
2.225329969703590564e-12 0.000000000000000000e+00 \\
3.712074117909949327e-12 0.000000000000000000e+00 \\
6.192112830212025429e-12 0.000000000000000000e+00 \\
1.032906673848005339e-11 0.000000000000000000e+00 \\
1.722992177523380047e-11 0.000000000000000000e+00 \\
2.874124176918251573e-11 0.000000000000000000e+00 \\
4.794328083497010580e-11 0.000000000000000000e+00 \\
7.997421251594699026e-11 0.000000000000000000e+00 \\
1.334050268600027960e-10 0.000000000000000000e+00 \\
2.225329969703590920e-10 0.000000000000000000e+00 \\
3.712074117909949650e-10 0.000000000000000000e+00 \\
6.192112830212009726e-10 9.000000000000000000e+00 \\
1.032906673848003633e-09 1.300000000000000000e+01 \\
1.722992177523380150e-09 1.430000000000000000e+02 \\
2.874124176918251780e-09 9.400000000000000000e+02 \\
4.794328083497010735e-09 7.414000000000000000e+03 \\
7.997421251594698199e-09 4.059300000000000000e+04 \\
1.334050268600027794e-08 4.359600000000000000e+04 \\
2.225329969703584995e-08 1.947000000000000000e+03 \\
3.712074117909943777e-08 1.201000000000000000e+03 \\
6.192112830212008568e-08 8.410000000000000000e+02 \\
1.032906673848003625e-07 5.900000000000000000e+02 \\
1.722992177523380448e-07 3.800000000000000000e+02 \\
2.874124176918251548e-07 2.620000000000000000e+02 \\
4.794328083497010669e-07 1.760000000000000000e+02 \\
7.997421251594698001e-07 1.040000000000000000e+02 \\
1.334050268600027847e-06 7.000000000000000000e+01 \\
2.225329969703585246e-06 5.700000000000000000e+01 \\
3.712074117909943380e-06 3.000000000000000000e+01 \\
6.192112830212009521e-06 2.200000000000000000e+01 \\
1.032906673848003662e-05 1.500000000000000000e+01 \\
1.722992177523380300e-05 1.000000000000000000e+01 \\
2.874124176918251570e-05 1.000000000000000000e+01 \\
4.794328083497011135e-05 6.000000000000000000e+00 \\
7.997421251594698255e-05 6.000000000000000000e+00 \\
1.334050268600027889e-04 0.000000000000000000e+00 \\
2.225329969703584857e-04 3.000000000000000000e+00 \\
3.712074117909933656e-04 2.000000000000000000e+00 \\
6.192112830212015721e-04 6.000000000000000000e+00 \\
1.032906673848005275e-03 8.000000000000000000e+00 \\
1.722992177523380124e-03 1.100000000000000000e+01 \\
2.874124176918244414e-03 3.700000000000000000e+01 \\
4.794328083497016203e-03 4.400000000000000000e+01 \\
7.997421251594711428e-03 8.500000000000000000e+01 \\
1.334050268600027803e-02 1.440000000000000000e+02 \\
2.225329969703584987e-02 2.370000000000000000e+02 \\
3.712074117909934523e-02 2.970000000000000000e+02 \\
6.192112830212015417e-02 3.260000000000000000e+02 \\
1.032906673848005275e-01 2.120000000000000000e+02 \\
1.722992177523380297e-01 1.130000000000000000e+02 \\
2.874124176918244622e-01 3.800000000000000000e+01 \\
4.794328083496991466e-01 2.000000000000000000e+00 \\
7.997421251594685199e-01 0.000000000000000000e+00 \\
1.334050268600027955e+00 0.000000000000000000e+00 \\
2.225329969703584876e+00 0.000000000000000000e+00 \\
3.712074117909933690e+00 0.000000000000000000e+00 \\
6.192112830212015417e+00 0.000000000000000000e+00 \\
1.032906673848005141e+01 0.000000000000000000e+00 \\
1.722992177523380164e+01 0.000000000000000000e+00 \\
2.874124176918244444e+01 0.000000000000000000e+00 \\
4.794328083496991155e+01 0.000000000000000000e+00 \\
7.997421251594685998e+01 0.000000000000000000e+00 \\
};
\addlegendentry{$(D,3,7)$}

\legend{}

\end{axis}

==> plot/C_P_0.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(0in,-0.12in)},
scale only axis,
xmin=0,
xmax=2,
%xlabel style={font=\color{white!15!black}, yshift=0.06in},
%xlabel={Point noise (px)},
label style={font=\small},
%title={$\sigma_v$ = 0$^{\circ}$},
ymin=0,
ymax=35,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.07in},
ylabel style={yshift=-0.15in, xshift=-0.03in},
ylabel={tr. err. ($^{\circ}$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
xticklabel=\empty
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 5.65598e-07 \\
0.1 6.42049 \\
0.2 9.30054 \\
0.3 11.5038 \\
0.4 13.1888 \\
0.5 14.5917 \\
0.6 15.641 \\
0.7 16.4253 \\
0.8 17.5906 \\
0.9 18.024 \\
1.0 18.8658 \\
1.1 19.3334 \\
1.2 20.1443 \\
1.3 20.7191 \\
1.4 20.6856 \\
1.5 21.2378 \\
1.6 21.8848 \\
1.7 22.1241 \\
1.8 22.722 \\
1.9 23.1292 \\
2.0 23.2129 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 6.12893e-07 \\
0.1 10.349 \\
0.2 14.4967 \\
0.3 17.0251 \\
0.4 19.1874 \\
0.5 20.4965 \\
0.6 21.9827 \\
0.7 22.8268 \\
0.8 23.9221 \\
0.9 24.8038 \\
1.0 25.4312 \\
1.1 25.9825 \\
1.2 26.7358 \\
1.3 27.1893 \\
1.4 27.6019 \\
1.5 28.184 \\
1.6 28.6093 \\
1.7 28.9214 \\
1.8 29.448 \\
1.9 29.4625 \\
2.0 30.0135 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.0467569 \\
0.1 5.58194 \\
0.2 6.76202 \\
0.3 7.30209 \\
0.4 7.71253 \\
0.5 8.12629 \\
0.6 8.2825 \\
0.7 8.63971 \\
0.8 8.74023 \\
0.9 8.87388 \\
1.0 8.92496 \\
1.1 9.14523 \\
1.2 9.26211 \\
1.3 9.32357 \\
1.4 8.98356 \\
1.5 9.29875 \\
1.6 9.42467 \\
1.7 9.57853 \\
1.8 9.59163 \\
1.9 9.64433 \\
2.0 9.61698 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.000000000000000000e+00 1.131000000000000005e+00 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}

==> plot/C_P_D.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(0.73in,-0.12in)},
scale only axis,
xmin=0,
xmax=2,
%xlabel style={font=\color{white!15!black}, yshift=0.06in},
%xlabel={Point noise (px)},
label style={font=\small},
%title={$\sigma_v$ = 0$^{\circ}$},
ymin=0,
ymax=35,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.07in},
ylabel style={yshift=-0.2in, xshift=-0.03in},
%ylabel={tr. err. ($^{\circ}$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
xticklabel=\empty,
yticklabel=\empty
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 7.43645 \\
0.1 9.87898 \\
0.2 11.7098 \\
0.3 13.7134 \\
0.4 14.6069 \\
0.5 16.0041 \\
0.6 16.6359 \\
0.7 17.6725 \\
0.8 18.5747 \\
0.9 19.0346 \\
1.0 19.4896 \\
1.1 20.2527 \\
1.2 20.4765 \\
1.3 21.3662 \\
1.4 21.4486 \\
1.5 22.1512 \\
1.6 22.7769 \\
1.7 22.4221 \\
1.8 22.9905 \\
1.9 23.5824 \\
2.0 23.3575 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 15.8311 \\
0.1 17.6084 \\
0.2 19.5143 \\
0.3 21.0648 \\
0.4 21.8905 \\
0.5 23.2817 \\
0.6 23.879 \\
0.7 24.9829 \\
0.8 25.4267 \\
0.9 26.0637 \\
1.0 26.8402 \\
1.1 27.4953 \\
1.2 27.7984 \\
1.3 27.9455 \\
1.4 28.3568 \\
1.5 28.864 \\
1.6 29.4057 \\
1.7 29.5645 \\
1.8 30.1325 \\
1.9 30.1451 \\
2.0 30.3088 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.882357 \\
0.1 5.82554 \\
0.2 6.63974 \\
0.3 7.54155 \\
0.4 7.78869 \\
0.5 7.99394 \\
0.6 8.18023 \\
0.7 8.78805 \\
0.8 8.72201 \\
0.9 8.90725 \\
1.0 8.99598 \\
1.1 9.4076 \\
1.2 9.2172 \\
1.3 9.28177 \\
1.4 9.36606 \\
1.5 9.32489 \\
1.6 9.34034 \\
1.7 9.33422 \\
1.8 9.58084 \\
1.9 9.57803 \\
2.0 9.73354 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.000000000000000000e+00 1.131000000000000005e+00 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}

==> plot/C_P_D_rebuttal.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.12\columnwidth,
at={(0.9in,0.389in)},
scale only axis,
xmin=0,
xmax=2,
xlabel style={font=\color{white!15!black}, yshift=0.07in},
xlabel={$\sigma_p$ (px)},
label style={font=\small},
title={tran err ($^\circ$)},
ymin=0,
ymax=20,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.07in},
ylabel style={yshift=-0.2in, xshift=-0.03in},
%ylabel={tr. err. ($^{\circ}$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
%xticklabel=\empty,
%yticklabel=\empty
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0		5.93941		\\
0.1		6.12506		\\
0.2		6.56896		\\
0.3		7.36289		\\
0.4		7.89556		\\
0.5		8.24955		\\
0.6		8.79032		\\
0.7		9.58201		\\
0.8		10.4268		\\
0.9		10.8545		\\
1		11.5394		\\
1.1		11.8705		\\
1.2		12.5944		\\
1.3		13.0421		\\
1.4		13.5135		\\
1.5		14.0689		\\
1.6		14.3684		\\
1.7		14.9129		\\
1.8		15.5485		\\
1.9		15.6799		\\
2		16.2577		\\
};
\addlegendentry{(E,3,5)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0		0.895344		\\
0.1		3.82221		\\
0.2		4.86806		\\
0.3		5.67198		\\
0.4		6.2175		\\
0.5		6.55072		\\
0.6		6.90529		\\
0.7		7.19871		\\
0.8		7.9757		\\
0.9		7.47266		\\
1		7.93824		\\
1.1		8.46245		\\
1.2		8.19507		\\
1.3		8.15832		\\
1.4		8.28902		\\
1.5		9.24939		\\
1.6		9.11266		\\
1.7		8.94457		\\
1.8		9.13053		\\
1.9		8.49983		\\
2		9.10401		\\
};
\addlegendentry{(D,3,7)}



\legend{}

\end{axis}

==> plot/C_V_0.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(1.46in,-0.12in)},
scale only axis,
xmin=0,
xmax=4,
%xlabel style={font=\color{white!15!black}, yshift=0.06in},
%xlabel={Point noise (px)},
label style={font=\small},
%title={$\sigma_v$ = 0$^{\circ}$},
ymin=0,
ymax=35,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.07in},
ylabel style={yshift=-0.2in, xshift=-0.03in},
%ylabel={tr. err. ($^{\circ}$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
xticklabel=\empty,
yticklabel=\empty
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 5.58627e-07 \\
0.2 2.69156 \\
0.4 4.20796 \\
0.6 5.60898 \\
0.8 6.66536 \\
1.0 7.47885 \\
1.2 8.2523 \\
1.4 9.16885 \\
1.6 9.641 \\
1.8 10.3335 \\
2.0 10.9173 \\
2.2 11.57 \\
2.4 11.892 \\
2.6 12.5463 \\
2.8 12.8484 \\
3.0 13.4739 \\
3.2 13.6481 \\
3.4 14.4772 \\
3.6 14.4802 \\
3.8 14.7754 \\
4.0 15.4064 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 6.11446e-07 \\
0.2 7.2258 \\
0.4 10.2764 \\
0.6 12.5697 \\
0.8 14.1913 \\
1.0 16.0442 \\
1.2 17.2188 \\
1.4 18.0321 \\
1.6 19.0461 \\
1.8 20.0292 \\
2.0 20.5526 \\
2.2 20.9472 \\
2.4 22.0809 \\
2.6 22.3918 \\
2.8 22.9504 \\
3.0 23.5148 \\
3.2 23.785 \\
3.4 24.0196 \\
3.6 24.5619 \\
3.8 25.0335 \\
4.0 25.4111 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.0555882 \\
0.2 0.330182 \\
0.4 0.493404 \\
0.6 0.682 \\
0.8 0.804501 \\
1.0 0.926875 \\
1.2 1.01541 \\
1.4 1.09104 \\
1.6 1.20856 \\
1.8 1.2514 \\
2.0 1.28813 \\
2.2 1.404 \\
2.4 1.5094 \\
2.6 1.51442 \\
2.8 1.58018 \\
3.0 1.68576 \\
3.2 1.73385 \\
3.4 1.77694 \\
3.6 1.84445 \\
3.8 1.88809 \\
4.0 1.89372 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.000000000000000000e+00 1.131000000000000005e+00 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}

==> plot/C_V_D.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(2.19in,-0.12in)},
scale only axis,
xmin=0,
xmax=4,
%xlabel style={font=\color{white!15!black}, yshift=0.06in},
%xlabel={Point noise (px)},
label style={font=\small},
%title={$\sigma_v$ = 0$^{\circ}$},
ymin=0,
ymax=35,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.07in},
ylabel style={yshift=-0.2in, xshift=-0.03in},
%ylabel={tr. err. ($^{\circ}$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
xticklabel=\empty,
yticklabel=\empty
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 18.6939 \\
0.2 18.7534 \\
0.4 18.9094 \\
0.6 19.2072 \\
0.8 19.3864 \\
1.0 19.7194 \\
1.2 19.974 \\
1.4 19.9072 \\
1.6 20.2158 \\
1.8 20.4661 \\
2.0 20.6094 \\
2.2 20.4678 \\
2.4 20.8918 \\
2.6 21.1198 \\
2.8 21.0469 \\
3.0 21.2495 \\
3.2 21.8078 \\
3.4 21.4747 \\
3.6 21.6399 \\
3.8 21.9631 \\
4.0 22.1006 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 25.6628 \\
0.2 25.8442 \\
0.4 25.7401 \\
0.6 25.7441 \\
0.8 26.4124 \\
1.0 26.47 \\
1.2 27.0281 \\
1.4 27.25 \\
1.6 27.2135 \\
1.8 27.6859 \\
2.0 27.8646 \\
2.2 28.1931 \\
2.4 28.2091 \\
2.6 28.5249 \\
2.8 28.5815 \\
3.0 28.9188 \\
3.2 29.1496 \\
3.4 29.2193 \\
3.6 29.4319 \\
3.8 29.7078 \\
4.0 29.7589 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 8.83804 \\
0.2 9.01502 \\
0.4 9.16005 \\
0.6 9.04319 \\
0.8 8.987 \\
1.0 8.93177 \\
1.2 9.17434 \\
1.4 9.15115 \\
1.6 8.98291 \\
1.8 9.03596 \\
2.0 9.18974 \\
2.2 9.07249 \\
2.4 9.05619 \\
2.6 9.1672 \\
2.8 8.94303 \\
3.0 9.11213 \\
3.2 9.11184 \\
3.4 9.27993 \\
3.6 8.92086 \\
3.8 9.12601 \\
4.0 9.14734 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.000000000000000000e+00 1.131000000000000005e+00 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}

==> plot/F_P_0.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(0in,-1.16in)},
scale only axis,
xmin=0,
xmax=2,
xlabel style={font=\color{white!15!black}, yshift=0.05in},
xlabel={$\sigma_p$ (px)},
label style={font=\small},
%title={$\sigma_v$ = 0$^{\circ}$},
ymin=0,
ymax=20,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.07in},
ylabel style={yshift=-0.15in, xshift=-0.17in},
ylabel={failures ($\%$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
ytick={0,10},
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.0 \\
0.1 6.507110000000001 \\
0.2 8.037519999999999 \\
0.3 9.13221 \\
0.4 10.0396 \\
0.5 10.1608 \\
0.6 10.770100000000001 \\
0.7 11.2058 \\
0.8 11.2058 \\
0.9 10.8973 \\
1.0 11.9718 \\
1.1 12.196 \\
1.2 11.197899999999999 \\
1.3 11.2767 \\
1.4 12.4956 \\
1.5 11.652999999999999 \\
1.6 12.0493 \\
1.7 11.933100000000001 \\
1.8 12.1574 \\
1.9 11.8787 \\
2.0 12.0338 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.0 \\
0.1 13.6666 \\
0.2 15.938099999999999 \\
0.3 16.5275 \\
0.4 17.0331 \\
0.5 17.6751 \\
0.6 16.7361 \\
0.7 17.2322 \\
0.8 17.163700000000002 \\
0.9 17.0056 \\
1.0 16.8745 \\
1.1 17.2322 \\
1.2 17.0262 \\
1.3 16.9228 \\
1.4 16.743 \\
1.5 16.7499 \\
1.6 16.1918 \\
1.7 16.4787 \\
1.8 16.0581 \\
1.9 16.6389 \\
2.0 17.3827 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.0 \\
0.1 7.86807 \\
0.2 8.5338 \\
0.3 8.79241 \\
0.4 9.20646 \\
0.5 9.420290000000001 \\
0.6 9.68208 \\
0.7 9.93425 \\
0.8 9.39567 \\
0.9 9.567730000000001 \\
1.0 9.03302 \\
1.1 10.0315 \\
1.2 9.420290000000001 \\
1.3 9.72285 \\
1.4 10.08 \\
1.5 9.55137 \\
1.6 9.608609999999999 \\
1.7 10.0558 \\
1.8 9.3135 \\
1.9 8.742469999999999 \\
2.0 9.42849 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.0 \\
0.1 0.0 \\
0.2 0.0 \\
0.3 0.0 \\
0.4 0.0 \\
0.5 0.0 \\
0.6 0.0 \\
0.7 0.0 \\
0.8 0.0 \\
0.9 0.0 \\
1.0 0.0 \\
1.1 0.0 \\
1.2 0.0 \\
1.3 0.0 \\
1.4 0.0 \\
1.5 0.0 \\
1.6 0.0 \\
1.7 0.0 \\
1.8 0.0 \\
1.9 0.0 \\
2.0 0.0 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}

==> plot/F_P_D.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(0.73in,-1.16in)},
scale only axis,
xmin=0,
xmax=2,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={$\sigma_p$ (px)},
label style={font=\small},
%title={$\sigma_v$ = 0$^{\circ}$},
ymin=0,
ymax=20,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.07in},
ylabel style={yshift=-0.2in, xshift=-0.1in},
%ylabel={failures ($\%$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
yticklabel=\empty,
ytick={0,10},
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 7.183960000000001 \\
0.1 9.1157 \\
0.2 9.94236 \\
0.3 10.2737 \\
0.4 10.4183 \\
0.5 10.793899999999999 \\
0.6 11.4417 \\
0.7 11.551400000000001 \\
0.8 11.8787 \\
0.9 12.273 \\
1.0 11.777700000000001 \\
1.1 11.8477 \\
1.2 12.5645 \\
1.3 11.5201 \\
1.4 12.640899999999998 \\
1.5 12.418999999999999 \\
1.6 11.902 \\
1.7 11.8632 \\
1.8 11.9951 \\
1.9 12.6866 \\
2.0 12.5874 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 16.36 \\
0.1 17.252799999999997 \\
0.2 17.519000000000002 \\
0.3 17.191100000000002 \\
0.4 17.0744 \\
0.5 18.1468 \\
0.6 17.6548 \\
0.7 17.2254 \\
0.8 17.553 \\
0.9 17.6209 \\
1.0 17.851 \\
1.1 17.0469 \\
1.2 17.3417 \\
1.3 16.631899999999998 \\
1.4 16.770699999999998 \\
1.5 16.7291 \\
1.6 16.8814 \\
1.7 17.0193 \\
1.8 17.2117 \\
1.9 15.909899999999999 \\
2.0 16.8952 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.0 \\
0.1 7.62978 \\
0.2 8.70081 \\
0.3 8.79241 \\
0.4 9.02475 \\
0.5 10.0153 \\
0.6 9.7147 \\
0.7 9.61678 \\
0.8 9.665759999999999 \\
0.9 10.249500000000001 \\
1.0 9.49407 \\
1.1 9.75544 \\
1.2 8.90873 \\
1.3 9.61678 \\
1.4 9.518640000000001 \\
1.5 9.37925 \\
1.6 9.29705 \\
1.7 9.48588 \\
1.8 9.52683 \\
1.9 9.403880000000001 \\
2.0 9.1157 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.0 \\
0.1 0.0 \\
0.2 0.0 \\
0.3 0.0 \\
0.4 0.0 \\
0.5 0.0 \\
0.6 0.0 \\
0.7 0.0 \\
0.8 0.0 \\
0.9 0.0 \\
1.0 0.0 \\
1.1 0.0 \\
1.2 0.0 \\
1.3 0.0 \\
1.4 0.0 \\
1.5 0.0 \\
1.6 0.0 \\
1.7 0.0 \\
1.8 0.0 \\
1.9 0.0 \\
2.0 0.0 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}

==> plot/F_P_D_rebuttal.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.12\columnwidth,
at={(1.8in,0.389in)},
scale only axis,
xmin=0,
xmax=2,
xlabel style={font=\color{white!15!black}, yshift=0.07in},
xlabel={$\sigma_p$ (px)},
label style={font=\small},
title={failures $\%$},
ymin=0,
ymax=10,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.07in},
ylabel style={yshift=-0.2in, xshift=-0.1in},
%ylabel={failures ($\%$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
%yticklabel=\empty
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0		5.60695		\\
0.1		5.63367		\\
0.2		5.92662		\\
0.3		6.55079		\\
0.4		6.21776		\\
0.5		6.26172		\\
0.6		6.41086		\\
0.7		6.55079		\\
0.8		6.6206		\\
0.9		7.22702		\\
1		7.38168		\\
1.1		7.44169		\\
1.2		7.12362		\\
1.3		7.82561		\\
1.4		7.91897		\\
1.5		8.24004		\\
1.6		7.88504		\\
1.7		8.24846		\\
1.8		8.28212		\\
1.9		7.81711		\\
2		8.48357		\\
};
\addlegendentry{(E,3,5)}


\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0		0		\\
0.1		4.67112		\\
0.2		5.03324		\\
0.3		6.32319		\\
0.4		5.39262		\\
0.5		6.62932		\\
0.6		6.67289		\\
0.7		5.83804		\\
0.8		7.14949		\\
0.9		6.62932		\\
1		6.97674		\\
1.1		6.32319		\\
1.2		6.67289		\\
1.3		8.04598		\\
1.4		8.13045		\\
1.5		7.32159		\\
1.6		7.62125		\\
1.7		7.70651		\\
1.8		8.71748		\\
1.9		7.49306		\\
2		8.59232		\\
};
\addlegendentry{(D,3,7)}



\legend{}

\end{axis}

==> plot/F_V_0.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(1.46in,-1.16in)},
scale only axis,
xmin=0,
xmax=4,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={$\sigma_v$ ($^{\circ}$)},
label style={font=\small},
%title={$\sigma_v$ = 0$^{\circ}$},
ymin=0,
ymax=20,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.07in},
ylabel style={yshift=-0.2in, xshift=-0.1in},
%ylabel={failures ($\%$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
yticklabel=\empty,
ytick={0,10},
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.0 \\
0.2 3.89236 \\
0.4 4.698370000000001 \\
0.6 6.076829999999999 \\
0.8 6.77729 \\
1.0 7.05456 \\
1.2 8.24846 \\
1.4 8.29895 \\
1.6 8.40813 \\
1.8 9.15698 \\
2.0 9.75544 \\
2.2 9.34639 \\
2.4 10.0558 \\
2.6 9.95047 \\
2.8 9.73915 \\
3.0 10.8655 \\
3.2 11.465300000000001 \\
3.4 11.4417 \\
3.6 11.7076 \\
3.8 11.777700000000001 \\
4.0 11.948599999999999 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.0 \\
0.2 11.7465 \\
0.4 13.1417 \\
0.6 14.8066 \\
0.8 15.860299999999999 \\
1.0 16.1144 \\
1.2 16.1707 \\
1.4 17.2939 \\
1.6 16.8468 \\
1.8 17.0469 \\
2.0 17.7158 \\
2.2 17.918400000000002 \\
2.4 16.8814 \\
2.6 17.824 \\
2.8 17.9723 \\
3.0 17.8577 \\
3.2 17.7632 \\
3.4 18.0126 \\
3.6 18.942999999999998 \\
3.8 18.507 \\
4.0 18.2405 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.0 \\
0.2 0.0 \\
0.4 0.0 \\
0.6 0.0 \\
0.8 0.0 \\
1.0 0.0 \\
1.2 0.0 \\
1.4 0.0 \\
1.6 0.0 \\
1.8 0.0 \\
2.0 0.0 \\
2.2 0.0 \\
2.4 0.0 \\
2.6 0.0 \\
2.8 0.0 \\
3.0 0.0 \\
3.2 0.0 \\
3.4 0.0 \\
3.6 0.0 \\
3.8 0.0 \\
4.0 0.0 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.0 \\
0.2 0.0 \\
0.4 0.0 \\
0.6 0.0 \\
0.8 0.0 \\
1.0 0.0 \\
1.2 0.0 \\
1.4 0.0 \\
1.6 0.0 \\
1.8 0.0 \\
2.0 0.0 \\
2.2 0.0 \\
2.4 0.0 \\
2.6 0.0 \\
2.8 0.0 \\
3.0 0.0 \\
3.2 0.0 \\
3.4 0.0 \\
3.6 0.0 \\
3.8 0.0 \\
4.0 0.0 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}

==> plot/F_V_D.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(2.19in,-1.16in)},
scale only axis,
xmin=0,
xmax=4,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={$\sigma_v$ ($^{\circ}$)},
label style={font=\small},
%title={$\sigma_v$ = 0$^{\circ}$},
ymin=0,
ymax=20,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.07in},
ylabel style={yshift=-0.2in, xshift=-0.1in},
%ylabel={failures ($\%$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
yticklabel=\empty,
ytick={0,10},
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 11.855400000000001 \\
0.2 12.080200000000001 \\
0.4 11.3711 \\
0.6 11.0558 \\
0.8 12.0493 \\
1.0 11.363199999999999 \\
1.2 12.0879 \\
1.4 12.4726 \\
1.6 11.9176 \\
1.8 12.3499 \\
2.0 12.6027 \\
2.2 12.709500000000002 \\
2.4 12.1265 \\
2.6 12.6332 \\
2.8 12.533900000000001 \\
3.0 12.648499999999999 \\
3.2 12.854 \\
3.4 12.740000000000002 \\
3.6 13.005700000000001 \\
3.8 13.5621 \\
4.0 12.701899999999998 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 16.9987 \\
0.2 17.191100000000002 \\
0.4 17.5802 \\
0.6 16.9021 \\
0.8 17.150000000000002 \\
1.0 16.6458 \\
1.2 17.3963 \\
1.4 17.627699999999997 \\
1.6 17.553 \\
1.8 17.1431 \\
2.0 16.9987 \\
2.2 17.566599999999998 \\
2.4 17.8577 \\
2.6 17.797 \\
2.8 17.1843 \\
3.0 18.2739 \\
3.2 17.5122 \\
3.4 17.8982 \\
3.6 17.884700000000002 \\
3.8 18.334 \\
4.0 17.369 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 9.80428 \\
0.2 9.559560000000001 \\
0.4 9.60043 \\
0.6 9.4367 \\
0.8 9.64944 \\
1.0 9.60043 \\
1.2 9.85306 \\
1.4 9.75544 \\
1.6 9.81241 \\
1.8 9.81241 \\
2.0 9.788 \\
2.2 9.8368 \\
2.4 10.2011 \\
2.6 9.81241 \\
2.8 9.84493 \\
3.0 9.86119 \\
3.2 10.1689 \\
3.4 9.77172 \\
3.6 9.64128 \\
3.8 9.4449 \\
4.0 9.477689999999999 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.0 \\
0.2 0.0 \\
0.4 0.0 \\
0.6 0.0 \\
0.8 0.0 \\
1.0 0.0 \\
1.2 0.0 \\
1.4 0.0 \\
1.6 0.0 \\
1.8 0.0 \\
2.0 0.0 \\
2.2 0.0 \\
2.4 0.0 \\
2.6 0.0 \\
2.8 0.0 \\
3.0 0.0 \\
3.2 0.0 \\
3.4 0.0 \\
3.6 0.0 \\
3.8 0.0 \\
4.0 0.0 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}

==> plot/R_P_0.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(0in,0.389in)},
scale only axis,
xmin=0,
xmax=2,
%xlabel style={font=\color{white!15!black}, yshift=0.06in},
%xlabel={Point noise (px)},
label style={font=\small},
title={$\sigma_v$ = 0$^{\circ}$},
ymin=0,
ymax=35,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
ylabel style={yshift=-0.15in, xshift=-0.0in},
ylabel={rot. err. ($^{\circ}$)},
grid=both,
legend style={at={(2.1,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
xticklabel=\empty
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 8.33742e-09 \\
0.1 1.93364 \\
0.2 2.81592 \\
0.3 3.46144 \\
0.4 3.87488 \\
0.5 4.3423 \\
0.6 4.66491 \\
0.7 4.89485 \\
0.8 5.17716 \\
0.9 5.31883 \\
1.0 5.46983 \\
1.1 5.67985 \\
1.2 5.84395 \\
1.3 6.03446 \\
1.4 6.05432 \\
1.5 6.10054 \\
1.6 6.3367 \\
1.7 6.41288 \\
1.8 6.68685 \\
1.9 6.67722 \\
2.0 6.65277 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 1.05837e-10 \\
0.1 3.3086 \\
0.2 4.747 \\
0.3 5.69345 \\
0.4 6.2401 \\
0.5 6.83663 \\
0.6 7.26535 \\
0.7 7.60861 \\
0.8 7.94166 \\
0.9 8.19274 \\
1.0 8.57975 \\
1.1 8.75266 \\
1.2 8.98024 \\
1.3 9.21237 \\
1.4 9.30681 \\
1.5 9.47668 \\
1.6 9.58091 \\
1.7 9.70248 \\
1.8 9.88575 \\
1.9 10.0236 \\
2.0 10.064 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.40801 \\
0.1 16.418 \\
0.2 20.4725 \\
0.3 21.6831 \\
0.4 23.6366 \\
0.5 24.8488 \\
0.6 25.8836 \\
0.7 26.611 \\
0.8 27.2327 \\
0.9 27.9601 \\
1.0 27.9216 \\
1.1 28.8402 \\
1.2 29.2195 \\
1.3 28.6457 \\
1.4 29.6464 \\
1.5 29.8138 \\
1.6 30.3685 \\
1.7 30.1238 \\
1.8 30.5646 \\
1.9 31.2704 \\
2.0 30.8385 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.000000000000000000e+00 1.131000000000000005e+00 \\
};
\addlegendentry{(B,3,7)}


%\legend{}

\end{axis}

==> plot/R_P_D.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(0.73in,0.389in)},
scale only axis,
xmin=0,
xmax=2,
%xlabel style={font=\color{white!15!black}, yshift=0.06in},
%xlabel={Point noise (px)},
label style={font=\small},
title={$\sigma_v$ = 1$^{\circ}$},
ymin=0,
ymax=35,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
ylabel style={yshift=-0.2in, xshift=-0.0in},
%ylabel={rot. err. ($^{\circ}$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
xticklabel=\empty,
yticklabel=\empty
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 2.92422 \\
0.1 3.57512 \\
0.2 4.13163 \\
0.3 4.54372 \\
0.4 4.93186 \\
0.5 5.15501 \\
0.6 5.43422 \\
0.7 5.6488 \\
0.8 5.73231 \\
0.9 6.06899 \\
1.0 6.35527 \\
1.1 6.32808 \\
1.2 6.45325 \\
1.3 6.71117 \\
1.4 6.76729 \\
1.5 7.00802 \\
1.6 7.01734 \\
1.7 7.12218 \\
1.8 7.08444 \\
1.9 7.28076 \\
2.0 7.3076 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 5.83221 \\
0.1 6.52259 \\
0.2 6.96478 \\
0.3 7.55388 \\
0.4 7.85409 \\
0.5 8.23329 \\
0.6 8.39739 \\
0.7 8.80165 \\
0.8 9.12059 \\
0.9 9.34807 \\
1.0 9.32438 \\
1.1 9.64744 \\
1.2 9.84708 \\
1.3 9.964 \\
1.4 10.0248 \\
1.5 10.055 \\
1.6 10.3179 \\
1.7 10.3579 \\
1.8 10.7497 \\
1.9 10.5748 \\
2.0 10.6572 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 3.45307 \\
0.1 17.5943 \\
0.2 20.3964 \\
0.3 22.7569 \\
0.4 24.2649 \\
0.5 25.0224 \\
0.6 25.9739 \\
0.7 26.8218 \\
0.8 27.191 \\
0.9 28.0808 \\
1.0 28.2372 \\
1.1 29.0772 \\
1.2 28.9696 \\
1.3 29.6584 \\
1.4 29.2051 \\
1.5 30.2836 \\
1.6 30.0977 \\
1.7 30.4394 \\
1.8 30.712 \\
1.9 30.7915 \\
2.0 31.2247 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.000000000000000000e+00 1.131000000000000005e+00 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}

==> plot/R_P_D_rebuttal.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.12\columnwidth,
at={(0in,0.389in)},
scale only axis,
xmin=0,
xmax=2,
%xlabel style={font=\color{white!15!black}, yshift=0.06in},
%xlabel={Point noise (px)},
xlabel style={font=\color{white!15!black}, yshift=0.07in},
xlabel={$\sigma_p$ (px)},
label style={font=\small},
title={rot err $(^\circ)$},
ymin=0,
ymax=30,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
ylabel style={yshift=-0.25in, xshift=-0.0in},
%ylabel={rot. err. ($^{\circ}$)},
grid=both,
legend style={at={(2.1,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
%xticklabel=\empty
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0		2.39604		\\
0.1		2.42962		\\
0.2		2.48727		\\
0.3		2.64728		\\
0.4		2.67841		\\
0.5		2.7768		\\
0.6		2.86692		\\
0.7		3.08277		\\
0.8		3.17369		\\
0.9		3.32852		\\
1		3.39167		\\
1.1		3.45313		\\
1.2		3.63976		\\
1.3		3.7518		\\
1.4		3.851		\\
1.5		3.99865		\\
1.6		4.0144		\\
1.7		4.21178		\\
1.8		4.29532		\\
1.9		4.35282		\\
2		4.47074		\\
};
\addlegendentry{(E,3,5)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0		3.55915		\\
0.1		10.7261		\\
0.2		13.1084		\\
0.3		15.0527		\\
0.4		16.7998		\\
0.5		16.9385		\\
0.6		19.036		\\
0.7		19.2931		\\
0.8		21.4387		\\
0.9		20.4707		\\
1		21.3724		\\
1.1		23.0063		\\
1.2		22.5138		\\
1.3		22.7666		\\
1.4		23.003		\\
1.5		24.7911		\\
1.6		25.6634		\\
1.7		24.5826		\\
1.8		23.5123		\\
1.9		24.3167		\\
2		25.1055		\\
};
\addlegendentry{(D,3,7)}


\legend{}

\end{axis}

==> plot/R_V_0.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(1.46in,0.389in)},
scale only axis,
xmin=0,
xmax=4,
%xlabel style={font=\color{white!15!black}, yshift=0.06in},
%xlabel={Point noise (px)},
label style={font=\small},
title={$\sigma_p$ = 0 px},
ymin=0,
ymax=35,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
ylabel style={yshift=-0.2in, xshift=-0.0in},
%ylabel={rot. err. ($^{\circ}$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
xticklabel=\empty,
yticklabel=\empty
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 2.28961e-09 \\
0.2 0.948509 \\
0.4 1.50669 \\
0.6 2.10102 \\
0.8 2.56761 \\
1.0 2.95538 \\
1.2 3.23441 \\
1.4 3.79475 \\
1.6 3.95043 \\
1.8 4.32446 \\
2.0 4.75663 \\
2.2 4.98585 \\
2.4 5.21726 \\
2.6 5.57275 \\
2.8 5.74439 \\
3.0 6.10935 \\
3.2 6.36939 \\
3.4 6.72242 \\
3.6 6.97835 \\
3.8 7.17274 \\
4.0 7.46364 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 2.79879e-10 \\
0.2 2.39396 \\
0.4 3.62971 \\
0.6 4.44161 \\
0.8 5.12207 \\
1.0 5.82839 \\
1.2 6.34323 \\
1.4 6.86412 \\
1.6 7.22428 \\
1.8 7.77855 \\
2.0 8.19681 \\
2.2 8.5079 \\
2.4 8.94909 \\
2.6 9.07315 \\
2.8 9.53395 \\
3.0 9.85372 \\
3.2 10.1504 \\
3.4 10.3073 \\
3.6 10.6335 \\
3.8 11.05 \\
4.0 11.259 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.408817 \\
0.2 1.41182 \\
0.4 1.95353 \\
0.6 2.56964 \\
0.8 3.13746 \\
1.0 3.54396 \\
1.2 3.89107 \\
1.4 4.41653 \\
1.6 4.78017 \\
1.8 5.30434 \\
2.0 5.38227 \\
2.2 5.82868 \\
2.4 6.33498 \\
2.6 6.4971 \\
2.8 6.93295 \\
3.0 7.33442 \\
3.2 7.50536 \\
3.4 8.00774 \\
3.6 8.4127 \\
3.8 8.62173 \\
4.0 8.81218 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.000000000000000000e+00 1.131000000000000005e+00 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}

==> plot/R_V_D.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(2.19in,0.389in)},
scale only axis,
xmin=0,
xmax=4,
%xlabel style={font=\color{white!15!black}, yshift=0.06in},
%xlabel={Point noise (px)},
label style={font=\small},
title={$\sigma_p$ = 1 px},
ymin=0,
ymax=35,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
ylabel style={yshift=-0.2in, xshift=-0.0in},
%ylabel={rot. err. ($^{\circ}$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
xticklabel=\empty,
yticklabel=\empty
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 5.59813 \\
0.2 5.56928 \\
0.4 5.64152 \\
0.6 5.90105 \\
0.8 6.04252 \\
1.0 6.31851 \\
1.2 6.38699 \\
1.4 6.47736 \\
1.6 6.81259 \\
1.8 6.94118 \\
2.0 7.16263 \\
2.2 7.16752 \\
2.4 7.63491 \\
2.6 7.69259 \\
2.8 7.87149 \\
3.0 8.03037 \\
3.2 8.22854 \\
3.4 8.48535 \\
3.6 8.67126 \\
3.8 8.85889 \\
4.0 9.03826 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 8.58475 \\
0.2 8.76032 \\
0.4 8.77756 \\
0.6 8.91958 \\
0.8 9.10242 \\
1.0 9.41117 \\
1.2 9.72512 \\
1.4 9.82268 \\
1.6 9.96083 \\
1.8 10.4676 \\
2.0 10.5587 \\
2.2 10.6088 \\
2.4 10.8402 \\
2.6 11.1304 \\
2.8 11.409 \\
3.0 11.5308 \\
3.2 11.7914 \\
3.4 11.9345 \\
3.6 12.028 \\
3.8 12.4905 \\
4.0 12.8238 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 27.4818 \\
0.2 28.1426 \\
0.4 28.2756 \\
0.6 28.1108 \\
0.8 28.4114 \\
1.0 28.6074 \\
1.2 28.479 \\
1.4 28.6474 \\
1.6 28.5586 \\
1.8 28.2509 \\
2.0 28.9383 \\
2.2 29.3134 \\
2.4 29.0917 \\
2.6 28.4391 \\
2.8 28.6922 \\
3.0 29.4202 \\
3.2 29.9924 \\
3.4 29.3676 \\
3.6 28.9537 \\
3.8 29.78 \\
4.0 29.5764 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.000000000000000000e+00 1.131000000000000005e+00 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}

==> plot/T_P_0.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(0in,-0.66in)},
scale only axis,
xmin=0,
xmax=2,
%xlabel style={font=\color{white!15!black}, yshift=0.06in},
%xlabel={Point noise (px)},
label style={font=\small},
%title={$\sigma_v$ = 0$^{\circ}$},
ymin=0,
ymax=1,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.07in},
ylabel style={yshift=-0.15in, xshift=-0.03in},
ylabel={ten. err. ($^{\circ}$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
xticklabel=\empty,
ytick={0,0.4,0.8},
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 1.2921e-12 \\
0.1 0.155082 \\
0.2 0.224425 \\
0.3 0.283629 \\
0.4 0.323952 \\
0.5 0.365736 \\
0.6 0.39343 \\
0.7 0.413986 \\
0.8 0.441551 \\
0.9 0.458611 \\
1.0 0.479287 \\
1.1 0.491466 \\
1.2 0.507756 \\
1.3 0.527413 \\
1.4 0.528432 \\
1.5 0.543566 \\
1.6 0.555198 \\
1.7 0.568493 \\
1.8 0.583939 \\
1.9 0.594478 \\
2.0 0.594542 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 3.62109e-12 \\
0.1 0.212511 \\
0.2 0.301503 \\
0.3 0.366082 \\
0.4 0.411619 \\
0.5 0.437821 \\
0.6 0.466384 \\
0.7 0.489991 \\
0.8 0.512717 \\
0.9 0.530077 \\
1.0 0.547698 \\
1.1 0.55827 \\
1.2 0.571279 \\
1.3 0.580411 \\
1.4 0.59026 \\
1.5 0.599129 \\
1.6 0.607331 \\
1.7 0.62242 \\
1.8 0.622364 \\
1.9 0.625296 \\
2.0 0.638795 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 5.59257e-11 \\
0.1 0.279411 \\
0.2 0.37622 \\
0.3 0.420354 \\
0.4 0.463807 \\
0.5 0.494271 \\
0.6 0.512687 \\
0.7 0.534852 \\
0.8 0.543995 \\
0.9 0.562084 \\
1.0 0.567821 \\
1.1 0.584 \\
1.2 0.600215 \\
1.3 0.60467 \\
1.4 0.60311 \\
1.5 0.618369 \\
1.6 0.626882 \\
1.7 0.628079 \\
1.8 0.633582 \\
1.9 0.635531 \\
2.0 0.640871 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 5.89179e-12 \\
0.1 0.364055 \\
0.2 0.482558 \\
0.3 0.545507 \\
0.4 0.600459 \\
0.5 0.644356 \\
0.6 0.671665 \\
0.7 0.698945 \\
0.8 0.707441 \\
0.9 0.727974 \\
1.0 0.740275 \\
1.1 0.763208 \\
1.2 0.77164 \\
1.3 0.783773 \\
1.4 0.792565 \\
1.5 0.799438 \\
1.6 0.806168 \\
1.7 0.812596 \\
1.8 0.827787 \\
1.9 0.828922 \\
2.0 0.837443 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}

==> plot/T_P_D.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(0.73in,-0.66in)},
scale only axis,
xmin=0,
xmax=2,
%xlabel style={font=\color{white!15!black}, yshift=0.06in},
%xlabel={Point noise (px)},
label style={font=\small},
%title={$\sigma_v$ = 0$^{\circ}$},
ymin=0,
ymax=1,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.07in},
ylabel style={yshift=-0.2in, xshift=-0.03in},
%ylabel={ten. err. ($^{\circ}$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
xticklabel=\empty,
yticklabel=\empty,
ytick={0,0.4,0.8},
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.175849 \\
0.1 0.242384 \\
0.2 0.289435 \\
0.3 0.341963 \\
0.4 0.364729 \\
0.5 0.396896 \\
0.6 0.422522 \\
0.7 0.444765 \\
0.8 0.464867 \\
0.9 0.488135 \\
1.0 0.499193 \\
1.1 0.51599 \\
1.2 0.524602 \\
1.3 0.546152 \\
1.4 0.554386 \\
1.5 0.569961 \\
1.6 0.580898 \\
1.7 0.581275 \\
1.8 0.593793 \\
1.9 0.607298 \\
2.0 0.602321 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.32301 \\
0.1 0.367014 \\
0.2 0.408801 \\
0.3 0.442454 \\
0.4 0.46864 \\
0.5 0.493752 \\
0.6 0.505055 \\
0.7 0.525693 \\
0.8 0.538742 \\
0.9 0.552097 \\
1.0 0.56281 \\
1.1 0.58157 \\
1.2 0.591365 \\
1.3 0.59304 \\
1.4 0.601607 \\
1.5 0.612603 \\
1.6 0.616453 \\
1.7 0.625395 \\
1.8 0.641081 \\
1.9 0.639934 \\
2.0 0.641525 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 5.63592e-11 \\
0.1 0.281855 \\
0.2 0.360654 \\
0.3 0.421298 \\
0.4 0.45942 \\
0.5 0.486793 \\
0.6 0.513376 \\
0.7 0.530375 \\
0.8 0.548903 \\
0.9 0.565278 \\
1.0 0.572196 \\
1.1 0.587852 \\
1.2 0.59355 \\
1.3 0.6034 \\
1.4 0.605206 \\
1.5 0.612863 \\
1.6 0.61306 \\
1.7 0.624897 \\
1.8 0.634675 \\
1.9 0.63438 \\
2.0 0.643767 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 1.33706e-11 \\
0.1 0.364425 \\
0.2 0.483375 \\
0.3 0.545171 \\
0.4 0.597827 \\
0.5 0.641572 \\
0.6 0.673805 \\
0.7 0.694933 \\
0.8 0.714735 \\
0.9 0.732781 \\
1.0 0.741438 \\
1.1 0.762716 \\
1.2 0.770351 \\
1.3 0.782503 \\
1.4 0.789983 \\
1.5 0.803089 \\
1.6 0.810632 \\
1.7 0.824432 \\
1.8 0.825974 \\
1.9 0.83753 \\
2.0 0.837346 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}

==> plot/T_V_0.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(1.46in,-0.66in)},
scale only axis,
xmin=0,
xmax=4,
%xlabel style={font=\color{white!15!black}, yshift=0.06in},
%xlabel={Point noise (px)},
label style={font=\small},
%title={$\sigma_v$ = 0$^{\circ}$},
ymin=0,
ymax=1,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.07in},
ylabel style={yshift=-0.2in, xshift=-0.03in},
%ylabel={ten. err. ($^{\circ}$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
xticklabel=\empty,
yticklabel=\empty,
ytick={0,0.4,0.8},
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 1.36693e-12 \\
0.2 0.0610855 \\
0.4 0.0952745 \\
0.6 0.129253 \\
0.8 0.157504 \\
1.0 0.176143 \\
1.2 0.196809 \\
1.4 0.221056 \\
1.6 0.232891 \\
1.8 0.253108 \\
2.0 0.269184 \\
2.2 0.286967 \\
2.4 0.296338 \\
2.6 0.311767 \\
2.8 0.317318 \\
3.0 0.33837 \\
3.2 0.348879 \\
3.4 0.369943 \\
3.6 0.373177 \\
3.8 0.377353 \\
4.0 0.391093 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 4.54494e-12 \\
0.2 0.142816 \\
0.4 0.206709 \\
0.6 0.257698 \\
0.8 0.292635 \\
1.0 0.33118 \\
1.2 0.354373 \\
1.4 0.374209 \\
1.6 0.39398 \\
1.8 0.415832 \\
2.0 0.430501 \\
2.2 0.438331 \\
2.4 0.458791 \\
2.6 0.468781 \\
2.8 0.483608 \\
3.0 0.490997 \\
3.2 0.500136 \\
3.4 0.501934 \\
3.6 0.5129 \\
3.8 0.520766 \\
4.0 0.529268 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 1.22956e-10 \\
0.2 5.03844e-11 \\
0.4 2.61815e-11 \\
0.6 1.50415e-11 \\
0.8 2.70983e-11 \\
1.0 9.54823e-11 \\
1.2 2.33439e-11 \\
1.4 5.55816e-11 \\
1.6 1.86578e-11 \\
1.8 2.61776e-11 \\
2.0 2.47586e-11 \\
2.2 2.14292e-11 \\
2.4 1.38114e-11 \\
2.6 2.11269e-11 \\
2.8 1.49455e-11 \\
3.0 3.58606e-11 \\
3.2 2.23229e-11 \\
3.4 1.50486e-10 \\
3.6 1.50304e-11 \\
3.8 1.07599e-11 \\
4.0 3.07726e-11 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 6.02298e-12 \\
0.2 1.0446e-11 \\
0.4 6.90504e-12 \\
0.6 2.26178e-11 \\
0.8 4.61403e-11 \\
1.0 1.23628e-11 \\
1.2 3.9738e-11 \\
1.4 2.50214e-11 \\
1.6 1.15047e-11 \\
1.8 5.27586e-12 \\
2.0 1.09964e-11 \\
2.2 7.10163e-12 \\
2.4 2.25404e-11 \\
2.6 1.98915e-11 \\
2.8 9.56071e-12 \\
3.0 8.77031e-12 \\
3.2 1.331e-11 \\
3.4 7.38281e-12 \\
3.6 9.83507e-12 \\
3.8 2.12924e-11 \\
4.0 1.36561e-11 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}

==> plot/T_V_D.tex <==
\begin{axis}[%
%xmode=log,
width=0.18\columnwidth,
height=0.13\columnwidth,
at={(2.19in,-0.66in)},
scale only axis,
xmin=0,
xmax=4,
%xlabel style={font=\color{white!15!black}, yshift=0.06in},
%xlabel={Point noise (px)},
label style={font=\small},
%title={$\sigma_v$ = 0$^{\circ}$},
ymin=0,
ymax=1,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.07in},
ylabel style={yshift=-0.2in, xshift=-0.03in},
%ylabel={ten. err. ($^{\circ}$)},
grid=both,
legend style={at={(2.3,1.45)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=4,
xticklabel=\empty,
yticklabel=\empty,
ytick={0,0.4,0.8},
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=red,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.474665 \\
0.2 0.475998 \\
0.4 0.479995 \\
0.6 0.489002 \\
0.8 0.494981 \\
1.0 0.50175 \\
1.2 0.507631 \\
1.4 0.512722 \\
1.6 0.52031 \\
1.8 0.528069 \\
2.0 0.528815 \\
2.2 0.528134 \\
2.4 0.543365 \\
2.6 0.545781 \\
2.8 0.55162 \\
3.0 0.55735 \\
3.2 0.568275 \\
3.4 0.565551 \\
3.6 0.567385 \\
3.8 0.579248 \\
4.0 0.58061 \\
};
\addlegendentry{(E,3,5)}

\addplot [color=green,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.544111 \\
0.2 0.555205 \\
0.4 0.549592 \\
0.6 0.552105 \\
0.8 0.558785 \\
1.0 0.55693 \\
1.2 0.570645 \\
1.4 0.569928 \\
1.6 0.580728 \\
1.8 0.58917 \\
2.0 0.591104 \\
2.2 0.596016 \\
2.4 0.597507 \\
2.6 0.607052 \\
2.8 0.607037 \\
3.0 0.611864 \\
3.2 0.617112 \\
3.4 0.61594 \\
3.6 0.620896 \\
3.8 0.627045 \\
4.0 0.629922 \\
};
\addlegendentry{(E,4,4)}

\addplot [color=blue,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.570311 \\
0.2 0.570671 \\
0.4 0.569705 \\
0.6 0.575003 \\
0.8 0.574385 \\
1.0 0.575257 \\
1.2 0.570827 \\
1.4 0.578488 \\
1.6 0.571648 \\
1.8 0.565885 \\
2.0 0.573816 \\
2.2 0.573528 \\
2.4 0.577164 \\
2.6 0.58054 \\
2.8 0.570538 \\
3.0 0.576043 \\
3.2 0.575758 \\
3.4 0.569233 \\
3.6 0.570779 \\
3.8 0.574554 \\
4.0 0.574675 \\
};
\addlegendentry{(D,3,7)}

\addplot [color=magenta,line width=1.3pt, mark options={solid, red}]  table[row sep=crcr]{%
0.0 0.746666 \\
0.2 0.750157 \\
0.4 0.743607 \\
0.6 0.753405 \\
0.8 0.750098 \\
1.0 0.741457 \\
1.2 0.746856 \\
1.4 0.750835 \\
1.6 0.744009 \\
1.8 0.749656 \\
2.0 0.749336 \\
2.2 0.750127 \\
2.4 0.749783 \\
2.6 0.745035 \\
2.8 0.745206 \\
3.0 0.748479 \\
3.2 0.754354 \\
3.4 0.749127 \\
3.6 0.746142 \\
3.8 0.743399 \\
4.0 0.742302 \\
};
\addlegendentry{(B,3,7)}


\legend{}

\end{axis}
